On the Globalization of ASPIN Employing Trust-Region Control Strategies -- Convergence Analysis and Numerical Examples

The parallel solution of large scale non-linear programming problems, which arise for example from the discretization of non-linear partial differential equations, is a highly demanding task. Here, a novel solution strategy is presented, which is inherently parallel and globally convergent. Each global non-linear iteration step consists of asynchronous solutions of local non-linear programming problems followed by a global recombination step. The recombination step, which is the solution of a quadratic programming problem, is designed in a way such that it ensures global convergence. As it turns out, the new strategy can be considered as a globalized additively preconditioned inexact Newton (ASPIN) method. However, in our approach the influence of ASPIN's non-linear preconditioner on the gradient is controlled in order to ensure a sufficient decrease condition. Two different control strategies are described and analyzed. Convergence to first-order critical points of our non-linear solution strategy is shown under standard trust-region assumptions. The strategy is investigated along difficult minimization problems arising from non-linear elasticity in 3D solved on a massively parallel computer with several thousand cores.

==> studies/cylinder128/stapelEps <==
set term postscript eps enhanced monochrome


set output "cylinder128-gradient.ps";
set grid;
set title "First-Order Sufficiency Conditions";

set xlabel "Performed Nonlinear Iterations";
set ylabel "Norm of the Gradient";

#set terminal png size 1024, 786;
set logscale y;

plot	"cylinder-2-ref-aptsTest-apts1-grids0-level2-128.txt" using 1:3 every 1 with linespoints title "Globalized Aspin", \
	"cylinder-2-ref-aptsTest-apts0-grids0-level2-128.txt" using 1:3 every 1 with linespoints title "Trust-Region";




set output "cylinder128-objectiveFunction.ps";
set grid;
set title "Objective Function";

set xlabel "Performed Nonlinear Iterations";
set ylabel "J(u)";

#set terminal png size 1024, 786;
unset logscale y;

plot	"cylinder-2-ref-aptsTest-apts1-grids0-level2-128.txt" using 1:2 with linespoints title "Globalized Aspin", \
	"cylinder-2-ref-aptsTest-apts0-grids0-level2-128.txt" using 1:2 with linespoints title "Trust-Region";





set output "cylinder128-trust-region.ps";
set grid;
set title "Trust-Region Radius";
set logscale y;
set xlabel "Performed Nonlinear Iterations";
set ylabel "{/Symbol D}_i";




plot	"cylinder-2-ref-aptsTest-apts1-grids0-level2-128.txt" using 1:4 with linespoints title "Globalized Aspin", \
	"cylinder-2-ref-aptsTest-apts0-grids0-level2-128.txt" using 1:4 with linespoints title "Trust-Region";



==> studies/massiveParallel/cylinder0121/stapelEps <==
set term postscript eps enhanced monochrome


set output "cylinder-firstOrder-240.ps";
set grid;
set title "First-Order Sufficiency Conditions";

set xlabel "Performed Nonlinear Iterations";
set ylabel "Norm of the Gradient";

#set terminal png size 1024, 786;
set logscale y;

plot	"cylinder-aptsTest-apts1-grids0-level2-240.txt" using 1:3 every 1 with linespoints title "Globalized Aspin", \
	"cylinder-aptsTest-apts0-grids0-level2-240.txt" using 1:3 every 1 with linespoints title "Trust-Region";




set output "cylinder-objectiveFunction-240.ps";
set grid;
set title "Objective Function";

set xlabel "Performed Nonlinear Iterations";
set ylabel "J(u)";

#set terminal png size 1024, 786;
unset logscale y;

plot	"cylinder-aptsTest-apts1-grids0-level2-240.txt" using 1:2 with linespoints title "Globalized Aspin", \
	"cylinder-aptsTest-apts0-grids0-level2-240.txt" using 1:2 with linespoints title "Trust-Region";





set output "cylinder-trust-region-240.ps";
set grid;
set title "Trust-Region Radius";
set logscale y;
set xlabel "Performed Nonlinear Iterations";
set ylabel "{/Symbol D}_i";




plot	"cylinder-aptsTest-apts1-grids0-level2-240.txt" using 1:4 with linespoints title "Globalized Aspin", \
	"cylinder-aptsTest-apts0-grids0-level2-240.txt" using 1:4 with linespoints title "Trust-Region";



==> studies/massiveParallel/sphere/stapelEps <==
set term postscript eps enhanced monochrome


set output "comparison-sphere-firstOrder.ps";
set grid;
set title "First-Order Sufficiency Conditions";

set xlabel "Performed Nonlinear Iterations";
set ylabel "Norm of the Gradient";

#set terminal png size 1024, 786;
set logscale y;
set yrange [1e-7:1000];
plot	"sphere-aptsTest-apts1-grids0-level2-240.txt" using 1:3 every 1 with linespoints title "Globalized Aspin   240 cores", \
	"sphere-aptsTest-apts1-grids0-level2-480.txt" using 1:3 every 1 with linespoints title "Globalized Aspin   480 cores", \
	"sphere-aptsTest-apts1-grids0-level2-920.txt" using 1:3 every 1 with linespoints title "Globalized Aspin   920 cores", \
	"sphere-aptsTest-apts1-grids0-level2-1840.txt" using 1:3 every 1 with linespoints title "Globalized Aspin 1,840 cores";




set output "comparison-sphere-objectiveFunction.ps";
set grid;
set title "Objective Function";

set xlabel "Performed Nonlinear Iterations";
set ylabel "J(u)";

#set terminal png size 1024, 786;
unset logscale y;

plot	"sphere-aptsTest-apts1-grids0-level2-240.txt" using 1:2 every 1 with linespoints title "Globalized Aspin   240 cores", \
	"sphere-aptsTest-apts1-grids0-level2-480.txt" using 1:2 every 1 with linespoints title "Globalized Aspin   480 cores", \
	"sphere-aptsTest-apts1-grids0-level2-920.txt" using 1:2 every 1 with linespoints title "Globalized Aspin   920 cores", \
	"sphere-aptsTest-apts1-grids0-level2-1840.txt" using 1:2 every 1 with linespoints title "Globalized Aspin 1,840 cores";





set output "comparison-sphere-trust-region.ps";
set grid;
set title "Trust-Region Radius";
set logscale y;
set xlabel "Performed Nonlinear Iterations";
set ylabel "{/Symbol D}_i";




plot	"sphere-aptsTest-apts1-grids0-level2-240.txt" using 1:4 every 1 with linespoints title "Globalized Aspin   240 cores", \
	"sphere-aptsTest-apts1-grids0-level2-480.txt" using 1:4 every 1 with linespoints title "Globalized Aspin   480 cores", \
	"sphere-aptsTest-apts1-grids0-level2-920.txt" using 1:4 every 1 with linespoints title "Globalized Aspin   920 cores", \
	"sphere-aptsTest-apts1-grids0-level2-1840.txt" using 1:4 every 1 with linespoints title "Globalized Aspin 1,840 cores";



==> studies/massiveParallel/sphere/stapelEpsTrAsp <==
set term postscript eps enhanced monochrome


set output "480sphere-firstOrder.ps";
set grid;
set title "First-Order Sufficiency Conditions";

set xlabel "Performed Nonlinear Iterations";
set ylabel "Norm of the Gradient";

#set terminal png size 1024, 786;
set logscale y;

plot	"sphere-aptsTest-apts1-grids0-level2-480.txt" using 1:3 every 1 with linespoints title "Globalized Aspin", \
	"sphere-aptsTest-apts0-grids0-level2-480.txt" using 1:3 every 1 with linespoints title "Trust-Region";




set output "480sphere-objectiveFunction.ps";
set grid;
set title "Objective Function";

set xlabel "Performed Nonlinear Iterations";
set ylabel "J(u)";

#set terminal png size 1024, 786;
unset logscale y;

plot	"sphere-aptsTest-apts1-grids0-level2-480.txt" using 1:2 with linespoints title "Globalized Aspin", \
	"sphere-aptsTest-apts0-grids0-level2-480.txt" using 1:2 with linespoints title "Trust-Region";





set output "480sphere-trust-region.ps";
set grid;
set title "Trust-Region Radius";
set logscale y;
set xlabel "Performed Nonlinear Iterations";
set ylabel "{/Symbol D}_i";




plot	"sphere-aptsTest-apts1-grids0-level2-480.txt" using 1:4 with linespoints title "Globalized Aspin", \
	"sphere-aptsTest-apts0-grids0-level2-480.txt" using 1:4 with linespoints title "Trust-Region";



==> studies/massiveParallel/stapelEps <==
set term postscript eps enhanced monochrome


set output "cylinder-firstOrder.ps";
set grid;
set title "First-Order Sufficiency Conditions";

set xlabel "Performed Nonlinear Iterations";
set ylabel "Norm of the Gradient";

#set terminal png size 1024, 786;
set logscale y;

plot	"cylinder-2-ref-aptsTest-apts1-grids0-level2-32.txt" using 1:3 every 1 with linespoints title "Globalized Aspin", \
	"cylinder-2-ref-aptsTest-apts0-grids0-level2-32.txt" using 1:3 every 1 with linespoints title "Trust-Region";




set output "cylinder-objectiveFunction.ps";
set grid;
set title "Objective Function";

set xlabel "Performed Nonlinear Iterations";
set ylabel "J(u)";

#set terminal png size 1024, 786;
unset logscale y;

plot	"cylinder-2-ref-aptsTest-apts1-grids0-level2-32.txt" using 1:2 with linespoints title "Globalized Aspin", \
	"cylinder-2-ref-aptsTest-apts0-grids0-level2-32.txt" using 1:2 with linespoints title "Trust-Region";





set output "cylinder-trust-region.ps";
set grid;
set title "Trust-Region Radius";
set logscale y;
set xlabel "Performed Nonlinear Iterations";
set ylabel "{/Symbol D}_i";




plot	"cylinder-2-ref-aptsTest-apts1-grids0-level2-32.txt" using 1:4 with linespoints title "Globalized Aspin", \
	"cylinder-2-ref-aptsTest-apts0-grids0-level2-32.txt" using 1:4 with linespoints title "Trust-Region";



==> studies/sphere32/stapelEps <==
set term postscript eps enhanced monochrome


set output "sphere-gradient32.ps";
set grid;
set title "First-Order Sufficiency Conditions";

set xlabel "Performed Nonlinear Iterations";
set ylabel "Norm of the Gradient";

#set terminal png size 1024, 786;
set logscale y;

plot	"ref-sphere-aptsTest-apts1-grids0-level2-32.txt" using 1:3 every 1 with linespoints title "Globalized Aspin", \
	"ref-sphere-aptsTest-apts0-grids0-level2-32.txt" using 1:3 every 1 with linespoints title "Trust-Region";




set output "sphere-objectiveFunction32.ps";
set grid;
set title "Objective Function";

set xlabel "Performed Nonlinear Iterations";
set ylabel "J(u)";

#set terminal png size 1024, 786;
unset logscale y;

plot	"ref-sphere-aptsTest-apts1-grids0-level2-32.txt" using 1:2 with linespoints title "Globalized Aspin", \
	"ref-sphere-aptsTest-apts0-grids0-level2-32.txt" using 1:2 with linespoints title "Trust-Region";





set output "sphere-trust-region32.ps";
set grid;
set title "Trust-Region Radius";
set logscale y;
set xlabel "Performed Nonlinear Iterations";
set ylabel "{/Symbol D}_i";




plot	"ref-sphere-aptsTest-apts1-grids0-level2-32.txt" using 1:4 with linespoints title "Globalized Aspin", \
	"ref-sphere-aptsTest-apts0-grids0-level2-32.txt" using 1:4 with linespoints title "Trust-Region";



==> studies/sphere64/stapelEps <==
set term postscript eps enhanced monochrome


set output "sphere-gradient64.ps";
set grid;
set title "First-Order Sufficiency Conditions";

set xlabel "Performed Nonlinear Iterations";
set ylabel "Norm of the Gradient";

#set terminal png size 1024, 786;
set logscale y;

plot	"ref-sphere-aptsTest-apts1-grids0-level2-64.txt" using 1:3 every 1 with linespoints title "Globalized Aspin", \
	"ref-sphere-aptsTest-apts0-grids0-level2-64.txt" using 1:3 every 1 with linespoints title "Trust-Region";




set output "sphere-objectiveFunction64.ps";
set grid;
set title "Objective Function";

set xlabel "Performed Nonlinear Iterations";
set ylabel "J(u)";

#set terminal png size 1024, 786;
unset logscale y;

plot	"ref-sphere-aptsTest-apts1-grids0-level2-64.txt" using 1:2 with linespoints title "Globalized Aspin", \
	"ref-sphere-aptsTest-apts0-grids0-level2-64.txt" using 1:2 with linespoints title "Trust-Region";





set output "sphere-trust-region64.ps";
set grid;
set title "Trust-Region Radius";
set logscale y;
set xlabel "Performed Nonlinear Iterations";
set ylabel "{/Symbol D}_i";




plot	"ref-sphere-aptsTest-apts1-grids0-level2-64.txt" using 1:4 with linespoints title "Globalized Aspin", \
	"ref-sphere-aptsTest-apts0-grids0-level2-64.txt" using 1:4 with linespoints title "Trust-Region";


